The LDBC Social Network Benchmark

The Linked Data Benchmark Council's Social Network Benchmark (LDBC SNB) is an effort intended to test various functionalities of systems used for graph-like data management. For this, LDBC SNB uses the recognizable scenario of operating a social network, characterized by its graph-shaped data. LDBC SNB consists of two workloads that focus on different functionalities: the Interactive workload (interactive transactional queries) and the Business Intelligence workload (analytical queries). This document contains the definition of both workloads. This includes a detailed explanation of the data used in the LDBC SNB, a detailed description for all queries, and instructions on how to generate the data and run the benchmark with the provided software.

==> Makefile <==
DOCUMENT=ldbc-snb-specification.tex

spec: $(DOCUMENT) choke-points/choke-points-queries.tex $(wildcard query-specifications/*.yaml)
	latexmk -pdf --interaction=batchmode $(DOCUMENT)

all: choke-points/choke-points-queries.tex query_cards workloads texfot
	ls *.pdf

choke-points/choke-points-queries.tex: $(wildcard query-specifications/*.yaml)
	./generate-tex.py

query_cards: $(DOCUMENT) choke-points/choke-points-queries.tex
	cd standalone-query-cards && \
	for card in *.tex; do \
		echo $$card ; \
		pdflatex --interaction=batchmode $$card ; \
		pdflatex --interaction=batchmode $$card ; \
	done

workloads: $(DOCUMENT) $(wildcard query-specifications/*.yaml)
	for doc in workload-*.tex; do \
		./texfot.pl latexmk -pdf --interaction=batchmode $$doc ; \
	done

texfot: $(DOCUMENT) choke-points/choke-points-queries.tex
	./texfot.pl latexmk -pdf --interaction=batchmode $(DOCUMENT)

clean:
	rm -f *.aux *.dvi *.thm *.lof *.log *.lot *.fls *.out *.toc *.bbl *.blg *.fdb_latexmk
	cd standalone-query-cards && rm -rf *.aux *.dvi *.thm *.lof *.log *.lot *.fls *.out *.toc *.bbl *.blg *.fdb_latexmk
	rm -f query-cards/*


==> development.tex <==
%%% DEVELOPMENT %%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Participation of Industry and Academia}

%\alert{List the significant entities that have influenced the development of the
%benchmark. Explain what advice/feedback that provided and show how this information
%helped to shape the current form of the benchmark.}

The broader dissemination policies include public relations by the LDBC
board (\eg press releases), the periodic progress
statements of task forces, and the TUC internal
and external (public) information, disseminated via
portals. LDBC also organizes events, mainly TUC
meetings\footnote{http://ldbc.eu:8090/display/TUC/Events}
where LDBC members meet the LDBC
audience (IT practitioners, researchers, industry).
Two of such TUC meetings were held already in
November 2012 and April 2013, with a third TUC
meeting coinciding with Neo Technology's Graph-Connect in London (November 19, 2013).
Additionally, LDBC sponsors and co-organizes scientific
workshops. In 2013, it organized the 1st International
workshop on Benchmarking RDF Systems
(BeRSys), co-located with ESWC'2013; and the 1st
International workshop on Graph Data Management
Experiences and Systems (GRADES), co-located with
SIGMOD/PODS 2013, as well as the GraphLab
2013 workshop held in San Francisco, an event
focusing on graph programming frameworks. Finally,
LDBC members publish technical aspects of benchmark
development in scientific literature~\cite{angles2013benchmarking,boncz2013tpch,cattuto2013time,gubichev2013sparqling}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\section{Changes of scope}

%\alert{When the scope of the benchmark was changed, either by increasing or decreasing
%the range of functionality tested, then details should be provided here with justifications.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\section{Significant deviations}

%\alert{Provide detail on any change of direction during the development phase.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> figures/fig-schema.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/schema-compact.pdf}
    \caption{%
    Partial LDBC social network schema depicted using a UML-like notation,
    focusing on the dynamic part of the graph (non-lifespan attributes and irrelevant entity types in the static part are omitted).
    %Only lifespan attributes (creation and deletion dates) are shown, other attributes are omitted. %(\eg Person's first name, birthday, \etc)
    In the dynamic part of the graph,
    all \emph{node types} and
    all $\otimes$~\emph{edge types with many-to-many cardinality between two dynamic node types} have individual lifespan attributes.
    The {\Large $\filleddiamond$}~\emph{containment edges} get their lifespan attributes from the contained endpoint (whose lifespan attributes are constrained by the container endpoint).
    $\oplus$~\tHasCreator follows the semantics of containment edges (even though it does not express an explicit containment relation).
    $\oast$~\tHasModerator is a one-to-many edge that is treated separately depending on the \tForum category (see \autoref{sec:hasModerator}).
    The $\odot$~\emph{edges between a dynamic and a static node} get their lifespan attributes from their dynamic endpoint.
    }
    \label{fig:schema}
\end{figure*}

==> short-descriptions/bi-read-01.tex <==
\paragraph{\textbf{Q1}. Posting summary.}
Given a \texttt{\$datetime}, find all \emph{Messages} created before
that moment. Group them by a 3-level grouping:
\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\tightlist
\item
  by year of creation
\item
  for each year, group into \emph{Message} types: is \emph{Comment} or
  not
\item
  for each year-type group, split into four groups based on length of
  their content
  \begin{itemize}
  \tightlist
  \item
    \texttt{0}: \(0 \leq \text{length} < 40\) (short)
  \item
    \texttt{1}: \(40 \leq \text{length} < 80\) (one liner)
  \item
    \texttt{2}: \(80 \leq \text{length} < 160\) (tweet)
  \item
    \texttt{3}: \(160 \leq \text{length}\) (long)
  \end{itemize}
\end{enumerate}


==> short-descriptions/bi-read-02.tex <==
\paragraph{\textbf{Q2}. Tag evolution.}
Find the \emph{Tags} under a given \texttt{\$tagClass} that were used in
\emph{Messages} during in the 100-day time window starting at
\texttt{\$date} and compare it with the 100-day time window that
follows. For the \emph{Tags} and for both time windows, compute the
count of \emph{Messages}.


==> short-descriptions/bi-read-03.tex <==
\paragraph{\textbf{Q3}. Popular topics in a country.}
Given a \texttt{\$tagClass} and a \texttt{\$country}, find all the
\emph{Forums} created in the given \texttt{\$country}, containing at
least one \emph{Message} with \emph{Tags} belonging directly to the
given \texttt{\$tagClass}, and count the \emph{Messages} by the
\emph{Forum} which contains them.
The location of a \emph{Forum} is identified by the location of the
\emph{Forum}'s moderator.


==> short-descriptions/bi-read-04.tex <==
\paragraph{\textbf{Q4}. Top message creators by country.}
Find the most popular \emph{Forums} by \emph{Country}, where the
popularity of a \emph{Forum} is measured by the number of members that
\emph{Forum} has from a given \emph{Country} and the \emph{Forum} was
created after a given \texttt{\$date}.
Calculate the top 100 most popular \emph{Forums}. If a \emph{Forum} is
popular in multiple countries, it should only be calculated once with
its largest membership. In case of a tie, the \emph{Forum} with the
smaller id value should be selected.
For each member \emph{Person} of the 100 most popular \emph{Forums},
count the number of \emph{Messages} (\texttt{messageCount}) they made in
any of those (most popular) \emph{Forums}. Also include those member
\emph{Persons} who have not posted any \emph{Messages} (have a
\texttt{messageCount} of 0).


==> short-descriptions/bi-read-05.tex <==
\paragraph{\textbf{Q5}. Most active posters of a given topic.}
Get each \emph{Person} (\texttt{person}) who has created a
\emph{Message} (\texttt{message}) with a given \texttt{\$tag} (direct
relation, not transitive). Considering only these \emph{Messages}, for
each \emph{Person}~node:
\begin{itemize}
\tightlist
\item
  Count its \emph{Messages} (\texttt{messageCount}).
\item
  Count \emph{likes} (\texttt{likeCount}) to its \emph{Messages}.
\item
  Count \emph{Comments} (\texttt{replyCount}) in reply to its
  \emph{Messages}.
\end{itemize}
The \texttt{score} is calculated according to the following formula:
\(1 \times \texttt{messageCount} + 2 \times \texttt{replyCount} + 10 \times \texttt{likeCount}\).


==> short-descriptions/bi-read-06.tex <==
\paragraph{\textbf{Q6}. Most authoritative users on a given topic.}
Given a \texttt{\$tag}, find all \emph{Persons} (\texttt{person1}) that
ever created a \emph{Message} with the \texttt{\$tag}. For each of these
\emph{Persons} (\texttt{person1}) compute their ``authority score'' as
follows:
\begin{itemize}
\tightlist
\item
  The ``authority score'' is the sum of ``popularity scores'' of the
  \emph{Persons} (\texttt{person2}) that liked any of that
  \emph{Person}'s \emph{Messages} with the given \texttt{\$tag} (same
  criterion as for \texttt{message1}).
\item
  A \emph{Person}'s (\texttt{person2}) ``popularity score'' is defined
  as the total number of likes (by any \emph{Person} \texttt{person3})
  on any of their \emph{Messages} (\texttt{message2}).
\end{itemize}


==> short-descriptions/bi-read-07.tex <==
\paragraph{\textbf{Q7}. Related topics.}
Find all \emph{Messages} that have a given \texttt{\$tag}. Find the
related \emph{Tags} attached to (direct) reply \emph{Comments} of these
\emph{Messages}, but only of those reply \emph{Comments} that do not
have the given \texttt{\$tag}.
Group the related \emph{Tags} by name, and get the count of replies in
each group.


==> short-descriptions/bi-read-08.tex <==
\paragraph{\textbf{Q8}. Central person for a tag.}
Given a \texttt{\$tag}, find all \emph{Persons} that are interested in
the \texttt{\$tag} and/or have written a \emph{Message} (\emph{Post} or
\emph{Comment}) with a \texttt{creationDate} after a given
\texttt{\$startDate} and that has a given \texttt{\$tag}. For each
\emph{Person}, compute the \texttt{score} as the sum of the following
two aspects:
\begin{itemize}
\tightlist
\item
  100, if the \emph{Person} has this \texttt{\$tag} as their interest,
  or 0 otherwise
\item
  number of \emph{Messages} by this \emph{Person} with the given
  \texttt{\$tag}
\end{itemize}
Also, for each \emph{Person}, compute the sum of the score of the
\emph{Person}'s friends (\texttt{friendsScore}).


==> short-descriptions/bi-read-09.tex <==
\paragraph{\textbf{Q9}. Top thread initiators.}
For each \emph{Person}, count the number of \emph{Posts} they created in
the time interval \texttt{{[}\$startDate,\ \$endDate{]}} (equivalent to
the number of threads they initiated) and the number of \emph{Messages}
in each of their (transitive) reply trees, including the root
\emph{Post} of each tree. When calculating \emph{Message} counts only
consider \emph{Messages} created within the given time interval.
Return each \emph{Person}, number of \emph{Posts} they created, and the
count of all \emph{Messages} that appeared in the reply trees (including
the \emph{Post} at the root of tree).


==> short-descriptions/bi-read-10.tex <==
\paragraph{\textbf{Q10}. Experts in social circle.}
Given a \emph{Person} \texttt{startPerson} with ID \texttt{\$personID},
find all other \emph{Persons} (\texttt{expertCandidatePerson}) that live
in a given \texttt{\$country} and are connected to the
\texttt{startPerson} on a \textbf{shortest path} with length in range
\texttt{{[}\$minPathDistance,\ \$maxPathDistance{]}} through the
\emph{knows} relation.
For each of these \texttt{expertCandidatePerson} nodes, retrieve all of
their \emph{Messages} that contain at least one \emph{Tag} belonging to
a given \texttt{\$tagClass} (direct relation not transitive). For each
\emph{Message}, retrieve all of its \emph{Tags}.
Group the results by \emph{Persons} and \emph{Tags}, then count the
\emph{Messages} by a certain \emph{Person} having a certain \emph{Tag}.


==> short-descriptions/bi-read-11.tex <==
\paragraph{\textbf{Q11}. Friend triangles.}
For a given \texttt{\$country}, count all the distinct triples of
\emph{Persons} such that:
\begin{itemize}
\tightlist
\item
  \texttt{personA} is friend of \texttt{personB},
\item
  \texttt{personB} is friend of \texttt{personC},
\item
  \texttt{personC} is friend of \texttt{personA},
\end{itemize}
and these friendships were created in the range
\texttt{{[}\$startDate,\ \$endDate{]}}.
Distinct means that given a triple \(t_1\) in the result set \(R\) of
all qualified triples, there is no triple \(t_2\) in \(R\) such that
\(t_1\) and \(t_2\) have the same set of elements.


==> short-descriptions/bi-read-12.tex <==
\paragraph{\textbf{Q12}. How many persons have a given number of messages.}
For each \emph{Person}, count the number of \emph{Messages} they made
(\texttt{messageCount}). Only count \emph{Messages} with the following
attributes:
\begin{itemize}
\item
  Its \texttt{content} is not empty (and consequently, the
  \texttt{imageFile} attribute is empty for \emph{Posts}).
\item
  Its \texttt{creationDate} is after \texttt{\$startDate} (exclusive,
  equality is not allowed).
\item
  Its \texttt{length} is below the \texttt{\$lengthThreshold}
  (exclusive, equality is not allowed).
\item
  It is written in any of the given \texttt{\$languages}.
  \begin{itemize}
  \tightlist
  \item
    The language of a \emph{Post} is defined by its \texttt{language}
    attribute.
  \item
    The language of a \emph{Comment} is that of the \emph{Post} that
    initiates the thread where the \emph{Comment} replies to.
  \end{itemize}
  The \emph{Post} and \emph{Comments} in the reply tree's path (from the
  \emph{Message} to the \emph{Post}) do not have to satisfy the
  constraints for \texttt{content}, \texttt{length}, and
  \texttt{creationDate}.
\end{itemize}
For each \texttt{messageCount} value, count the number of \emph{Persons}
with exactly \texttt{messageCount} \emph{Messages} (with the required
attributes).


==> short-descriptions/bi-read-13.tex <==
\paragraph{\textbf{Q13}. Zombies in a country.}
Find zombies within the given \texttt{\$country}, and return their
zombie scores. A \texttt{zombie} is a \emph{Person} created before the
given \texttt{\$endDate}, which has created an average of
\texttt{{[}0,\ 1)} \emph{Messages} per month, during the time range
between profile's \texttt{creationDate} and the given
\texttt{\$endDate}. The number of months spans the time range from the
\texttt{creationDate} of the profile to the \texttt{\$endDate} with
partial months on both end counting as one month (e.g.~a
\texttt{creationDate} of Jan 31 and an \texttt{\$endDate} of Mar 1
result in 3 months).
For each \texttt{zombie}, calculate the following:
\begin{itemize}
\tightlist
\item
  \texttt{zombieLikeCount}: the number of \emph{likes} received from
  other zombies.
\item
  \texttt{totalLikeCount}: the total number of \emph{likes} received.
\item
  \texttt{zombieScore}: \texttt{zombieLikeCount} /
  \texttt{totalLikeCount}. If the value of \texttt{totalLikeCount} is 0,
  the \texttt{zombieScore} of the \texttt{zombie} should be 0.0.
\end{itemize}
For both \texttt{zombieLikeCount} and \texttt{totalLikeCount}, only
consider \emph{likes} received from profiles that were created before
the given \texttt{\$endDate}.


==> short-descriptions/bi-read-14.tex <==
\paragraph{\textbf{Q14}. International dialog.}
Consider all pairs of people \texttt{(person1,\ person2)} such that (1)
they know each other, (2) one is located in a \emph{City} of
\texttt{\$country1}, and (3) the other is located in a \emph{City} of
\texttt{\$country2}. For each \emph{City} of \texttt{\$country1}, return
the highest scoring pair. If there are multiple top-scoring pairs in a
city, return the pair with the lowest (\texttt{person1.id},
\texttt{person2.id}) using a lexicographical ordering.
The score of a pair is defined as the sum of the subscores awarded for
the following kinds of interaction. The initial value is
\texttt{score\ =\ 0}.
\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\tightlist
\item
  \texttt{person1} has created a reply \emph{Comment} to at least one
  \emph{Message} by \texttt{person2}: \texttt{score\ +=\ 4}
\item
  \texttt{person1} has created at least one \emph{Message} that
  \texttt{person2} has created a reply to: \texttt{score\ +=\ 1}
\item
  \texttt{person1} liked at least one \emph{Message} by
  \texttt{person2}: \texttt{score\ +=\ 10}
\item
  \texttt{person1} has created at least one \emph{Message} that was
  liked by \texttt{person2}: \texttt{score\ +=\ 1}
\end{enumerate}
Consequently, the maximum score a pair can obtain is:
\texttt{4\ +\ 1\ +\ 10\ +\ 1\ =\ 16}.


==> short-descriptions/bi-read-15.tex <==
\paragraph{\textbf{Q15}. Trusted connection paths through forums created in a given timeframe.}
Given two \emph{Persons} with IDs \texttt{\$person1Id} and
\texttt{\$person2Id}, calculate the cost of the weighted shortest path
between these two \emph{Persons}, in the subgraph induced by the
\emph{knows} relationship. The interaction score of a \emph{knows} edge
is calculated based on the interactions of its \emph{Person} endpoints:
\begin{itemize}
\tightlist
\item
  Every direct reply (by one of the \emph{Persons}) to a \emph{Post} (by
  the other \emph{Person}) is 1.0 point.
\item
  Every direct reply (by one of the \emph{Persons}) to a \emph{Comment}
  (by the other \emph{Person}) is 0.5 points.
\end{itemize}
Only consider \emph{Messages} that were created in a \emph{Forum} that
was created within the timeframe (interval)
\texttt{{[}\$startDate,\ \$endDate{]}}. Note that for \emph{Comments},
the containing \emph{Forum} is that of the \emph{Post} that the comment
(transitively) replies to. Also note that interactions are counted both
ways.
The weight for the shortest path algorithm is determined as
\(\frac{1}{\textit{interaction score} + 1}\).
The result of the query is a single number, the cost of the weighted
shortest path. If no such path exists, the query should return \(-1.0\).


==> short-descriptions/bi-read-16.tex <==
\paragraph{\textbf{Q16}. Fake news detection.}
Given two \emph{Tag}/date pairs (\texttt{\$tagA}/\texttt{\$dateA} and
\texttt{\$tagB}/\texttt{\$dateB}), for each pair
\texttt{\$tagX}/\texttt{\$dateX}:
\begin{itemize}
\tightlist
\item
  Create an induced subgraph between \emph{Persons} where for each pair
  of \emph{Persons} \texttt{person1}/\texttt{person2}, both have created
  a \emph{Message} on the day of \texttt{\$dateX} with \emph{Tag}
  \texttt{\$tagX}.
\item
  In the induced subgraph, only keep pairs of \emph{Persons} who have at
  most \texttt{maxKnowsLimit} friends (in the induced subgraph).
\item
  For these \emph{Persons}, count the number of \emph{Messages} created
  on \texttt{\$dateX} with \emph{Tag} \texttt{\$tagX}.
\end{itemize}
Return \emph{Persons} who had at least one \emph{Messages} for both
\texttt{\$tagA}/\texttt{\$dateA} and \texttt{\$tagB}/\texttt{\$dateB}
ranked by their total number of \emph{Messages} (descending).


==> short-descriptions/bi-read-17.tex <==
\paragraph{\textbf{Q17}. Information propagation analysis.}
This query aims to identify instances of ``information propagation''
when a \emph{Person} (\texttt{person1}) submits a \emph{Message}
(\texttt{message1}) with a given \texttt{\$tag} to a \emph{Forum}
(\texttt{forum1}). This is read by other members of \texttt{forum1},
\emph{Persons} \texttt{person2} and \texttt{person3} (who must be
different \emph{Persons}). Some time later (specified by the
\texttt{\$delta} parameter), these persons have a discussion with the
same \texttt{\$tag} in a different \emph{Forum} (\texttt{forum2}) where
\texttt{person1} is not a member. The discussion consists of a
\emph{Message} (\texttt{message2}) by \texttt{person2} and a direct
reply \emph{Comment} (\texttt{comment}) by \texttt{person3}.
Return IDs of \texttt{person1} with the number of interactions their
\emph{Messages} (might have) caused.


==> short-descriptions/bi-read-18.tex <==
\paragraph{\textbf{Q18}. Friend recommendation.}
For a given \texttt{\$tag}, for each \texttt{person1} interested in
\texttt{\$tag}, recommend new friends (\texttt{person2}) who
\begin{itemize}
\tightlist
\item
  do not yet know \texttt{person1}
\item
  have at least one mutual friend with \texttt{person1}
\item
  are also interested in \texttt{\$tag}.
\end{itemize}
Rank \emph{Persons} \texttt{person2} based on the number of mutual
friends with \texttt{person1}.


==> short-descriptions/bi-read-19.tex <==
\paragraph{\textbf{Q19}. Interaction path between cities.}
Given two \emph{Cities} with IDs \texttt{\$city1Id}, \texttt{\$city2Id},
find \emph{Persons} \texttt{person1}, \texttt{person2} living in these
\emph{Cities} (respectively) with the \textbf{cheapest} interaction path
between them.
The cheapest path is equivalent to the \textbf{weighted shortest} path.
It is computed on a subgraph of the \emph{Person-knows-Person} graph
with the edge weights based on the number of interactions. An
\textbf{interaction} is a direct reply \emph{Comments} from one
\emph{Person} to \emph{Messages} by the other \emph{Person}. Only
\emph{knows} edges with at least one interaction between their endpoint
\emph{Persons} are considered. For these, the weight of a \emph{knows}
edge is defined as:
\(\max(\mathrm{round}( 40 - \sqrt{\textit{numInteractions}} ), 1)\)
If there are multiple pairs of people with cheapest paths that have the
same total weight, return all of them.
\textbf{Note:} Interactions are counted both ways, e.g.~if Alice
\emph{knows} Bob, Alice writes 2 reply \emph{Comments} to Bob's
\emph{Messages} and Bob writes 3 reply \emph{Comments} to Alice's
\emph{Messages}, their total number of interactions is 5 and the weight
of the knows edge is 38.
\textbf{Remark:} Determinism is ensured by using square root followed by
rounding. For all integers between 1 and \(\numprint{100000}\), the
square root's fractional part is more than 10e-5 from 0.5, where the
rounding could be non-determinstic based on floating point inaccuracies.
As 10e-5 is significantly larger than the machine epsilon of IEEE 754
floats (both 32- and 64-bit), the floating point inaccuracies have no
chance to affect the derived integer edge weights.


==> short-descriptions/bi-read-20.tex <==
\paragraph{\textbf{Q20}. Recruitment.}
Consider \emph{knows} edges where the endpoint \emph{Persons} attended
the same \emph{University} and set the weight of the edge to the
absolute difference between the year of enrolment plus 1. If the
\emph{Persons} attended multiple universities, we select the smallest
(\texttt{min}) value. Formally: \[
w = \min_{\textsf{studyAt}_\textsf{A}, \textsf{studyAt}_\textsf{B}}
  \left|
    \textsf{studyAt}_\textsf{A}.\textsf{classYear} -
    \textsf{studyAt}_\textsf{B}.\textsf{classYear}
  \right|
  + 1
\]
Given a \texttt{\$company} and a \emph{Person} \texttt{person2} with ID
\texttt{\$person2Id} (who is not working and has not worked at
\texttt{\$company}), find a different \emph{Person} (\texttt{person1})
who works or at some point worked in \texttt{\$company} and is reachable
from \texttt{person2} through people who have studied together through
the shortest weighted path.
If there are multiple \emph{Person} \texttt{person1} nodes with the same
shortest path length, return all of them.


==> short-descriptions/delete-01.tex <==
\paragraph{\textbf{Q1}. Remove person and its personal forums and message (sub)threads.}
Remove a \emph{Person} with ID \texttt{\$personId} and its edges
(\emph{isLocatedIn}, \emph{studyAt}, \emph{workAt}, \emph{hasInterest},
\emph{likes}, \emph{knows}, \emph{hasMember}, \emph{hasModerator},
\emph{hasCreator}). Additionally, remove the Album and Wall
\emph{Forums} whose moderator is the \emph{Person} and remove all
\emph{Messages} the \emph{Person} has created in the rest of the
\emph{Forums} (Groups).


==> short-descriptions/delete-02.tex <==
\paragraph{\textbf{Q2}. Remove post like.}
Given a \emph{Person} with ID \texttt{\$personId} and a \emph{Post} with
ID \texttt{\$postId}, remove the \emph{likes} edge between them.


==> short-descriptions/delete-03.tex <==
\paragraph{\textbf{Q3}. Remove comment like.}
Given a \emph{Person} with ID \texttt{\$personId} and a \emph{Comment}
with ID \texttt{\$commentId}, remove the \emph{likes} edge between them.


==> short-descriptions/delete-04.tex <==
\paragraph{\textbf{Q4}. Remove forum and its content.}
Remove a \emph{Forum} with ID \texttt{\$forumId} and its edges
(\emph{hasModerator}, \emph{hasMember}, \emph{hasTag}) and all
\emph{Posts} in the \emph{Forum} (connected by \emph{containerOf} edges)
and their direct and transitive \emph{Comments}.


==> short-descriptions/delete-05.tex <==
\paragraph{\textbf{Q5}. Remove forum membership.}
Given a \emph{Forum} with ID \texttt{\$forumId} and a \emph{Person} with
ID \texttt{\$personId}, remove the \emph{hasMember} edge between them.


==> short-descriptions/delete-06.tex <==
\paragraph{\textbf{Q6}. Remove post thread.}
Remove a \emph{Post} node with ID \texttt{\$postId} and its edges
(\emph{isLocatedIn}, \emph{likes}, \emph{hasCreator}, \emph{hasTag},
\emph{containerOf}). Remove all replies to the \emph{Post} and the
connecting \emph{replyOf} edges. In addition, remove all transitive
reply \emph{Comments} to the \emph{Post} and their edges.


==> short-descriptions/delete-07.tex <==
\paragraph{\textbf{Q7}. Remove comment subthread.}
Remove a \emph{Comment} node with ID \texttt{\$commentId} and its
\textbf{edges} (\emph{isLocatedIn}, \emph{likes}, \emph{hasCreator},
\emph{hasTag}). In addition, remove all replies to the \emph{Comment}
connected by \emph{replyOf} and their \textbf{edges}.


==> short-descriptions/delete-08.tex <==
\paragraph{\textbf{Q8}. Remove friendship.}
Given two \emph{Person} nodes with IDs \texttt{\$person1Id} and
\texttt{\$person2Id}, remove the \emph{knows} edge between them.


==> short-descriptions/insert-01.tex <==
\paragraph{\textbf{Q1}. Add person.}
Add a \emph{Person} \textbf{node}, connected to the network by 4
possible \textbf{edge} types.


==> short-descriptions/insert-02.tex <==
\paragraph{\textbf{Q2}. Add like to post.}
Add a \emph{likes} \textbf{edge} to a \emph{Post}.


==> short-descriptions/insert-03.tex <==
\paragraph{\textbf{Q3}. Add like to comment.}
Add a \emph{likes} \textbf{edge} to a \emph{Comment}.


==> short-descriptions/insert-04.tex <==
\paragraph{\textbf{Q4}. Add forum.}
Add a \emph{Forum} \textbf{node}, connected to the network by 2 possible
\textbf{edge} types.


==> short-descriptions/insert-05.tex <==
\paragraph{\textbf{Q5}. Add forum membership.}
Add a \emph{Forum} membership \textbf{edge} (\emph{hasMember}) to a
\emph{Person}.


==> short-descriptions/insert-06.tex <==
\paragraph{\textbf{Q6}. Add post.}
Add a \emph{Post} \textbf{node} connected to the network by 4 possible
\textbf{edge} types (\emph{hasCreator}, \emph{containerOf},
\emph{isLocatedIn}, \emph{hasTag}).


==> short-descriptions/insert-07.tex <==
\paragraph{\textbf{Q7}. Add comment.}
Add a \emph{Comment} \textbf{node} replying to a
\emph{Post}/\emph{Comment}, connected to the network by 4 possible
\textbf{edge} types (\emph{replyOf}, \emph{hasCreator},
\emph{isLocatedIn}, \emph{hasTag}).


==> short-descriptions/insert-08.tex <==
\paragraph{\textbf{Q8}. Add friendship.}
Add a friendship \textbf{edge} (\emph{knows}) between two
\emph{Persons}.


==> short-descriptions/interactive-complex-read-01.tex <==
\paragraph{\textbf{Q1}. Transitive friends with a certain name.}
Given a start \emph{Person} with ID \texttt{\$personId}, find
\emph{Persons} with a given first name (\texttt{\$firstName}) that the
start \emph{Person} is connected to (excluding start \emph{Person}) by
at most 3 steps via the \emph{knows} relationships. Return
\emph{Persons}, including the distance (1..3), summaries of the
\emph{Persons} workplaces and places of study.


==> short-descriptions/interactive-complex-read-02.tex <==
\paragraph{\textbf{Q2}. Recent messages by your friends.}
Given a start \emph{Person} with ID \texttt{\$personId}, find the most
recent \emph{Messages} from all of that \emph{Person}'s friends
(\texttt{friend} nodes). Only consider \emph{Messages} created before
the given \texttt{\$maxDate} (excluding that day).


==> short-descriptions/interactive-complex-read-03.tex <==
\paragraph{\textbf{Q3}. Friends and friends of friends that have been to given countries.}
Given a start \emph{Person} with ID \texttt{\$personId}, find
\emph{Persons} that are their friends and friends of friends (excluding
the start \emph{Person}) that have made \emph{Posts} / \emph{Comments}
in both of the given \emph{Countries} (named \texttt{\$countryXName} and
\texttt{\$countryYName}), within
\texttt{{[}\$startDate,\ \$startDate\ +\ \$durationDays)} (closed-open
interval). Only \emph{Persons} that are foreign to these
\emph{Countries} are considered, that is \emph{Persons} whose location
\emph{Country} is neither named \texttt{\$countryXName} nor
\texttt{\$countryYName}.


==> short-descriptions/interactive-complex-read-04.tex <==
\paragraph{\textbf{Q4}. New topics.}
Given a start \emph{Person} with ID \texttt{\$personId}, find
\emph{Tags} that are attached to \emph{Posts} that were created by that
\emph{Person}'s friends. Only include \emph{Tags} that were attached to
friends' \emph{Posts} created within a given time interval
\texttt{{[}\$startDate,\ \$startDate\ +\ \$durationDays)} (closed-open)
and that were never attached to friends' \emph{Posts} created before
this interval.


==> short-descriptions/interactive-complex-read-05.tex <==
\paragraph{\textbf{Q5}. New groups.}
Given a start \emph{Person} with ID \texttt{\$personId}, denote their
friends and friends of friends (excluding the start \emph{Person}) as
\texttt{otherPerson}.
Find \emph{Forums} that any \emph{Person} \texttt{otherPerson} became a
\emph{member} of after a given date (\texttt{\$minDate}). For each of
those \emph{Forums}, count the number of \emph{Posts} that were created
by the \emph{Person} \texttt{otherPerson}.


==> short-descriptions/interactive-complex-read-06.tex <==
\paragraph{\textbf{Q6}. Tag co-occurrence.}
Given a start \emph{Person} with ID \texttt{\$personId} and a \emph{Tag}
with name \texttt{\$tagName}, find the other \emph{Tags} that occur
together with this \emph{Tag} on \emph{Posts} that were created by start
\emph{Person}'s friends and friends of friends (excluding start
\emph{Person}). Return top 10 \emph{Tags}, and the count of \emph{Posts}
that were created by these \emph{Persons}, which contain both this
\emph{Tag} and the given \emph{Tag}.


==> short-descriptions/interactive-complex-read-07.tex <==
\paragraph{\textbf{Q7}. Recent likers.}
Given a start \emph{Person} with ID \texttt{\$personId}, find the most
recent \texttt{likes} on any of start \emph{Person}'s \emph{Messages}.
Find \emph{Persons} that liked (\texttt{likes} edge) any of start
\emph{Person}'s \emph{Messages}, the \emph{Messages} they liked most
recently, the creation date of that like, and the latency in minutes
(\texttt{minutesLatency}) between creation of \emph{Messages} and like.
Additionally, for each \emph{Person} found return a flag indicating
(\texttt{isNew}) whether the liker is a friend of start \emph{Person}.
In case that a \emph{Person} liked multiple \emph{Messages} at the same
time, return the \emph{Message} with lowest identifier.
\textbf{Validation rule:} Depending on whether the system-under-test
supports leap seconds or uses UTC-SLS (UTC with Smoothed Leap Seconds),
a difference of 1 minute can occur between the \texttt{minutesLatency}
results of two correct implementations when the time interval includes
June 30, 2012, when there was a leap second. Therefore, the
\texttt{minutesLatency} value is validated using a tolerance of 1
minute.


==> short-descriptions/interactive-complex-read-08.tex <==
\paragraph{\textbf{Q8}. Recent replies.}
Given a start \emph{Person} with ID \texttt{\$personId}, find the most
recent \emph{Comments} that are replies to \emph{Messages} of the start
\emph{Person}. Only consider direct (single-hop) replies, not the
transitive (multi-hop) ones. Return the reply \emph{Comments}, and the
\emph{Person} that created each reply \emph{Comment}.


==> short-descriptions/interactive-complex-read-09.tex <==
\paragraph{\textbf{Q9}. Recent messages by friends or friends of friends.}
Given a start \emph{Person} with ID \texttt{\$personId}, find the most
recent \emph{Messages} created by that \emph{Person}'s friends or
friends of friends (excluding the start \emph{Person}). Only consider
\emph{Messages} created before the given \texttt{\$maxDate} (excluding
that day).


==> short-descriptions/interactive-complex-read-10.tex <==
\paragraph{\textbf{Q10}. Friend recommendation.}
Given a start \emph{Person} with ID \texttt{\$personId}, find that
\emph{Person}'s friends of friends (\texttt{foaf}) -- excluding the
start \emph{Person} and his/her immediate friends --, who were born on
or after the 21st of a given \texttt{\$month} (in any year) and before
the 22nd of the following month. Calculate the similarity between each
\texttt{friend} and the start \texttt{person}, where
\texttt{commonInterestScore} is defined as follows:
\begin{itemize}
\tightlist
\item
  \texttt{common} = number of \emph{Posts} created by \texttt{friend},
  such that the \emph{Post} has a \emph{Tag} that the start
  \texttt{person} is interested in
\item
  \texttt{uncommon} = number of \emph{Posts} created by \texttt{friend},
  such that the \emph{Post} has no \emph{Tag} that the start
  \texttt{person} is interested in
\item
  \texttt{commonInterestScore} = \texttt{common} - \texttt{uncommon}
\end{itemize}


==> short-descriptions/interactive-complex-read-11.tex <==
\paragraph{\textbf{Q11}. Job referral.}
Given a start \emph{Person} with ID \texttt{\$personId}, find that
\emph{Person}'s friends and friends of friends (excluding start
\emph{Person}) who started working in some \emph{Company} in a given
\emph{Country} with name \texttt{\$countryName}, before a given date
(\texttt{\$workFromYear}).


==> short-descriptions/interactive-complex-read-12.tex <==
\paragraph{\textbf{Q12}. Expert search.}
Given a start \emph{Person} with ID \texttt{\$personId}, find the
\emph{Comments} that this \emph{Person}'s friends made in reply to
\emph{Posts}, considering only those \emph{Comments} that are direct
(single-hop) replies to \emph{Posts}, not the transitive (multi-hop)
ones. Only consider \emph{Posts} with a \emph{Tag} in a given
\emph{TagClass} with name \texttt{\$tagClassName} or in a descendent of
that \emph{TagClass}. Count the number of these reply \emph{Comments},
and collect the \emph{Tags} that were attached to the \emph{Posts} they
replied to, but only collect \emph{Tags} with the given \emph{TagClass}
or with a descendant of that \emph{TagClass}. Return \emph{Persons} with
at least one reply, the reply count, and the collection of \emph{Tags}.


==> short-descriptions/interactive-complex-read-13.tex <==
\paragraph{\textbf{Q13}. Single shortest path.}
Given two \emph{Persons} with IDs \texttt{\$person1Id} and
\texttt{\$person2Id}, find the shortest path between these two
\emph{Persons} in the subgraph induced by the \emph{knows} edges. Return
the length of this path:
\begin{itemize}
\tightlist
\item
  \(-1\): no path found
\item
  \(0\): start person = end person
\item
  \(> 0\): path found (start person \(\neq\) end person)
\end{itemize}


==> short-descriptions/interactive-complex-read-14-v1.tex <==
\paragraph{\textbf{Q14v1}. Trusted connection paths (v1).}
\textbf{This query is used in SNB Interactive v1.}
Given two \emph{Persons} with IDs \texttt{\$person1Id} and
\texttt{\$person2Id}, find all (unweighted) shortest paths between these
two \emph{Persons}, in the subgraph induced by the \emph{knows}
relationship.
Then, for each path calculate a weight. The nodes in the path are
\emph{Persons}, and the weight of a path is the sum of weights between
every pair of consecutive \emph{Person} nodes in the path.
The weight for a pair of \emph{Persons} is calculated based on their
interactions:
\begin{itemize}
\tightlist
\item
  Every direct reply (by one of the \emph{Persons}) to a \emph{Post} (by
  the other \emph{Person}) is 1.0.
\item
  Every direct reply (by one of the \emph{Persons}) to a \emph{Comment}
  (by the other \emph{Person}) is 0.5.
\end{itemize}
Note that interactions are counted both ways (e.g.~if Alice writes 2
\emph{Post} replies and 1 \emph{Comment} reply to Bob, while Bob writes
3 \emph{Post} replies and 4 \emph{Comment} replies to Alice, their
interaction score is
\(2 \times 1.0 + 1 \times 0.5 + 3 \times 1.0 + 4 \times 0.5 = 7.5\)).
Return all the paths with shortest length and their weights. Do not
return any rows if there is no path between the two \emph{Persons}.


==> short-descriptions/interactive-complex-read-14-v2.tex <==
\paragraph{\textbf{Q14v2}. Trusted connection paths (v2).}
\textbf{This query is used in SNB Interactive v2.}
Find a cheapest path between two given \emph{Persons} with IDs
\texttt{\$person1Id} and \texttt{\$person2Id} in the interaction
subgraph. If there are multiple cheapest paths, any of them can be
returned. Do not return any rows if there is no path between the
\emph{Persons}. The interaction subgraph is based on a projection of the
\emph{Person}-\emph{knows}-\emph{Person} graph. In this projection, only
those \emph{knows} edges are kept whose endpoint \emph{Persons} have at
least one interaction between them. An interaction is defined as a
direct reply \emph{Comment} (by one of the \emph{Persons}) to a
\emph{Message} (by the other \emph{Person}). The weights are defined as:
\(\max(\mathrm{round}( 40 - \sqrt{\textit{numInteractions}} ), 1)\)
\textbf{Note:} Interactions are counted both ways, e.g.~if Alice
\emph{knows} Bob, Alice writes 2 reply \emph{Comments} to Bob's
\emph{Messages} and Bob writes 3 reply \emph{Comments} to Alice's
\emph{Messages}, their total number of interactions is 5 and the weight
of the knows edge is 38.
\textbf{Remark:} Determinism is ensured by using square root followed by
rounding. For all integers between 1 and \(\numprint{100000}\), the
square root's fractional part is more than 10e-5 from 0.5, where the
rounding could be non-deterministic based on floating point
inaccuracies. As 10e-5 is significantly larger than the machine epsilon
of IEEE 754 floats (both 32- and 64-bit), the floating point
inaccuracies have no chance to affect the derived integer edge weights.


==> short-descriptions/interactive-short-read-01.tex <==
\paragraph{\textbf{Q1}. Profile of a person.}
Given a start \emph{Person} with ID \texttt{\$personId}, retrieve their
first name, last name, birthday, IP address, browser, and city of
residence.


==> short-descriptions/interactive-short-read-02.tex <==
\paragraph{\textbf{Q2}. Recent messages of a person.}
Given a start \emph{Person} with ID \texttt{\$personId}, retrieve the
last 10 \emph{Messages} created by that user. For each \emph{Message},
return that \emph{Message}, the original \emph{Post} in its conversation
(\texttt{post}), and the author of that \emph{Post}
(\texttt{originalPoster}). If any of the \emph{Messages} is a
\emph{Post}, then the original \emph{Post} (\texttt{post}) will be the
same \emph{Message}, i.e.~that \emph{Message} will appear twice in that
result.


==> short-descriptions/interactive-short-read-03.tex <==
\paragraph{\textbf{Q3}. Friends of a person.}
Given a start \emph{Person} with ID \texttt{\$personId}, retrieve all of
their friends, and the date at which they became friends.


==> short-descriptions/interactive-short-read-04.tex <==
\paragraph{\textbf{Q4}. Content of a message.}
Given a \emph{Message} with ID \texttt{\$messageId}, retrieve its
content and creation date.


==> short-descriptions/interactive-short-read-05.tex <==
\paragraph{\textbf{Q5}. Creator of a message.}
Given a \emph{Message} with ID \texttt{\$messageId}, retrieve its
author.


==> short-descriptions/interactive-short-read-06.tex <==
\paragraph{\textbf{Q6}. Forum of a message.}
Given a \emph{Message} with ID \texttt{\$messageId}, retrieve the
\emph{Forum} that contains it and the \emph{Person} that moderates that
\emph{Forum}. Since \emph{Comments} are not directly contained in
\emph{Forums}, for \emph{Comments}, return the \emph{Forum} containing
the original \emph{Post} in the thread which the \emph{Comment} is
replying to.


==> short-descriptions/interactive-short-read-07.tex <==
\paragraph{\textbf{Q7}. Replies of a message.}
Given a \emph{Message} with ID \texttt{\$messageId}, retrieve the
(1-hop) \emph{Comments} that reply to it.
In addition, return a boolean flag \texttt{knows} indicating if the
author of the reply (\texttt{replyAuthor}) knows the author of the
original message (\texttt{messageAuthor}). If author is same as original
author, return \texttt{False} for \texttt{knows} flag.


==> templates/choke-point-template.tex <==
\paragraph{Queries}
{\raggedright
{% for query in queries -%}
    \queryRefCard{ {{- query.0 -}} }{
      {%- if query.1 == "Interactive" and query.2 == "complex" -%}
        IC
      {%- elif query.1 == "BI" and query.2 == "read" -%}
        BI
      {%- elif query.2 == "insert" -%}
      INS
      {%- elif query.2 == "delete" -%}
        DEL
      {%- endif -%}
    }{ {{- query.3 -}} }
{% endfor -%}
{# this newline is required by \raggedright to work #}
}


==> templates/choke-points-queries.tex <==
% Template-based generation of the table showing choke point coverage by queries.
% Note that 'update' queries (DEL, INS) and their choke points (CP-9.x) are omitted from the table
\begin{table}[htbp]
\scriptsize
\centering
\begin{tabular}{|l|
    {%- for choke_point in choke_points -%}
        {% if choke_points[loop.index0 - 1][0] != choke_points[loop.index0][0] %}|{% endif %}c|
    {%- endfor -%}
} \hline
{% for choke_point in choke_points -%}
    {%- if choke_point < "9" -%}
        & \chokePoint{ {{- choke_point -}} }
    {%- endif -%}
{% endfor %} \\ \hline

{%- for query in queries -%}
    {#- only list queries that have at least one choke point -#}
    {%- if query_choke_point[query.0] and query.2 != "insert" and query.2 != "delete" -%}
        {%- if queries[loop.index0 - 1].0[0] != queries[loop.index0].0[0] %}\hline{% endif %}
        \queryRefCard{ {{- query.0 -}} }{
            {%- if query.1 == "Interactive" and query.2 == "complex"%}IC{% endif -%}
            {%- if query.1 == "BI" and query.2 == "read"%}BI{% endif -%}
            }{ {{- query.3 -}} }
        {% for choke_point in choke_points -%}
            {%- if choke_point < "9" -%}
                & {% if choke_point in query_choke_point[query.0] %} \yes {%- else %} {% endif %}
            {%- endif -%}
        {% endfor %} \\ \hline
    {%- endif -%}
{% endfor %}

\end{tabular}
\caption{Coverage of choke points by queries.}
\label{tab:query_choke_point}
\end{table}


==> templates/query-card-template.tex <==
\renewcommand*{\arraystretch}{1.1}

\subsection*{ {{- workload }} / {{ operation }} / {{ number -}} }
\label{sec: {{- query_id -}} }

% change \emph{} to use sans-serif font
\let\oldemph\emph
\renewcommand{\emph}[1]{{ '{{' }}\footnotesize \sf #1}}
\let\oldtextbf\textbf
\renewcommand{\textbf}[1]{{ '{{' }}\it #1}}

{%- if workload == "Interactive" and operation == "complex" -%}
\renewcommand{\currentQueryCard}{ {{- query_id -}} }
\marginpar{
	\raggedleft
	\vspace{0.22ex}

	\queryRefCard{interactive-complex-read-01}{IC}{1}\\
	\queryRefCard{interactive-complex-read-02}{IC}{2}\\
	\queryRefCard{interactive-complex-read-03}{IC}{3}\\
	\queryRefCard{interactive-complex-read-04}{IC}{4}\\
	\queryRefCard{interactive-complex-read-05}{IC}{5}\\
	\queryRefCard{interactive-complex-read-06}{IC}{6}\\
	\queryRefCard{interactive-complex-read-07}{IC}{7}\\
	\queryRefCard{interactive-complex-read-08}{IC}{8}\\
	\queryRefCard{interactive-complex-read-09}{IC}{9}\\
	\queryRefCard{interactive-complex-read-10}{IC}{10}\\
	\queryRefCard{interactive-complex-read-11}{IC}{11}\\
	\queryRefCard{interactive-complex-read-12}{IC}{12}\\
	\queryRefCard{interactive-complex-read-13}{IC}{13}\\
	\queryRefCard{interactive-complex-read-14-v1}{IC}{14v1}\\
	\queryRefCard{interactive-complex-read-14-v2}{IC}{14v2}\\
}
{%- endif %}

{%- if workload == "Interactive" and operation == "short" -%}
\renewcommand{\currentQueryCard}{ {{- query_id -}} }
\marginpar{
	\raggedleft
	\vspace{0.22ex}

	\queryRefCard{interactive-short-read-01}{IS}{1}\\
	\queryRefCard{interactive-short-read-02}{IS}{2}\\
	\queryRefCard{interactive-short-read-03}{IS}{3}\\
	\queryRefCard{interactive-short-read-04}{IS}{4}\\
	\queryRefCard{interactive-short-read-05}{IS}{5}\\
	\queryRefCard{interactive-short-read-06}{IS}{6}\\
	\queryRefCard{interactive-short-read-07}{IS}{7}\\
}
{%- endif %}

{% if workload == "BI" and operation == "read" -%}
\renewcommand{\currentQueryCard}{ {{- query_id -}} }
\marginpar{
	\vspace{0.22ex}
	\raggedleft

	\queryRefCard{bi-read-01}{BI}{1}\\
	\queryRefCard{bi-read-02}{BI}{2}\\
	\queryRefCard{bi-read-03}{BI}{3}\\
	\queryRefCard{bi-read-04}{BI}{4}\\
	\queryRefCard{bi-read-05}{BI}{5}\\
	\queryRefCard{bi-read-06}{BI}{6}\\
	\queryRefCard{bi-read-07}{BI}{7}\\
	\queryRefCard{bi-read-08}{BI}{8}\\
	\queryRefCard{bi-read-09}{BI}{9}\\
	\queryRefCard{bi-read-10}{BI}{10}\\
	\queryRefCard{bi-read-11}{BI}{11}\\
	\queryRefCard{bi-read-12}{BI}{12}\\
	\queryRefCard{bi-read-13}{BI}{13}\\
	\queryRefCard{bi-read-14}{BI}{14}\\
	\queryRefCard{bi-read-15}{BI}{15}\\
	\queryRefCard{bi-read-16}{BI}{16}\\
	\queryRefCard{bi-read-17}{BI}{17}\\
	\queryRefCard{bi-read-18}{BI}{18}\\
	\queryRefCard{bi-read-19}{BI}{19}\\
	\queryRefCard{bi-read-20}{BI}{20}\\
}
{% endif -%}

{%- if operation == "insert" -%}
\renewcommand{\currentQueryCard}{ {{- query_id -}} }
\marginpar{
	\raggedleft
	\vspace{0.22ex}

	\queryRefCard{insert-01}{INS}{1}\\
	\queryRefCard{insert-02}{INS}{2}\\
	\queryRefCard{insert-03}{INS}{3}\\
	\queryRefCard{insert-04}{INS}{4}\\
	\queryRefCard{insert-05}{INS}{5}\\
	\queryRefCard{insert-06}{INS}{6}\\
	\queryRefCard{insert-07}{INS}{7}\\
	\queryRefCard{insert-08}{INS}{8}\\
}
{%- endif %}

{%- if operation == "delete" -%}
\renewcommand{\currentQueryCard}{ {{- query_id -}} }
\marginpar{
	\raggedleft
	\vspace{0.22ex}

	\queryRefCard{delete-01}{DEL}{1}\\
	\queryRefCard{delete-02}{DEL}{2}\\
	\queryRefCard{delete-03}{DEL}{3}\\
	\queryRefCard{delete-04}{DEL}{4}\\
	\queryRefCard{delete-05}{DEL}{5}\\
	\queryRefCard{delete-06}{DEL}{6}\\
	\queryRefCard{delete-07}{DEL}{7}\\
	\queryRefCard{delete-08}{DEL}{8}\\
}
{%- endif %}

\noindent\begin{tabularx}{\queryCardWidth}{|>{\queryPropertyCell}p{\queryPropertyCellWidth}|X|}
	\hline
	query & {{ workload }} / {{ operation }} / {{ number }} \\ \hline
%
	title & {{ title }} \\ \hline
%
	pattern & \centering \includegraphics[scale=\patternscale,margin=0cm .2cm]{patterns/{{ query_id -}} } \tabularnewline \hline
%
	description & {{ description }} \\ \hline
%
	{% if parameters %}
		params &
		\innerCardVSpace{\begin{tabularx}{\attributeCardWidth}{|>{\paramNumberCell}C{\attributeNumberWidth}|>{\varNameCell}M|>{\typeCell}m{\typeWidth}|Y|} \hline
		{% for entry in parameters -%}
			$\mathsf{ {{- loop.index -}} }$ & \${{ entry.name }} & {{ entry.type }} & {{ entry.description }} \\ \hline
		{% endfor -%}
		\end{tabularx}}\innerCardVSpace \\ \hline
	{% endif %}
%
	{% if result %}
		result &
		\innerCardVSpace{\begin{tabularx}{\attributeCardWidth}{|>{\resultNumberCell}C{\attributeNumberWidth}|>{\varNameCell}M|>{\typeCell}m{\typeWidth}|>{\resultOriginCell}c|Y|} \hline
		{% for entry in result -%}
			$\mathsf{ {{- loop.index -}} }$ & {{ entry.name|trim() }} & {{ entry.type|trim() }} & {% set cat = entry.category|trim() -%}
					{%- if   cat == "aggregated" -%} A
					{%- elif cat == "calculated" -%} C
					{%- elif cat == "meta" -%} M
					{%- else -%} R
					{%- endif %} &
				{{ entry.description }} \\ \hline
		{% endfor -%}
		\end{tabularx}}\innerCardVSpace \\ \hline
	{% endif %}
%
	{% if sort %}
		sort		&
		\innerCardVSpace{\begin{tabularx}{\attributeCardWidth}{|>{\sortNumberCell}C{\attributeNumberWidth}|>{\varNameCell}M|>{\directionCell}c|Y|} \hline
		{% for entry in sort -%}
			$\mathsf{ {{- loop.index -}} }$ & {{ entry.name }} & $\{{ entry.direction }}$ & {{ entry.description }} \\ \hline
		{% endfor -%}
		\end{tabularx}}\innerCardVSpace \\ \hline
	{% endif -%}
%
	{% if limit -%}
		limit & {{ limit }} \\ \hline
	{% endif -%}
%
	{% if choke_points -%}
	CPs &
	\multicolumn{1}{>{\raggedright}l|}{
		{% for choke_point in choke_points -%}
			\chokePoint{ {{- choke_point -}} } {%- if not loop.last %}, {% endif %}
		{% endfor -%}
	} \\ \hline
	{% endif -%}
%
	{% if relevance -%}
	relevance &
		\footnotesize {{ relevance }} \\ \hline
	{%- endif -%}
%
\end{tabularx}
\queryCardVSpace

% change \emph and \textbf back to the old ones
\let\emph\oldemph
\let\textbf\oldtextbf

\renewcommand{\currentQueryCard}{0}


==> templates/short-description-template.tex <==
\paragraph{\textbf{Q {{- number }}}. {{ title }}.}

{{ description }}

